From Text to Discovery: How Large Language Models Are Reshaping Research Across Scientific and Humanistic Disciplines

Large Language Models (LLMs) are rapidly reshaping academic research across the natural sciences, social sciences, and humanities, yet the scientific community lacks a comprehensive, cross-disciplinary account of how these tools are being integrated, what they deliver, and where they fall short. This paper addresses that gap by mapping their current state and outlining an agenda for their responsible integration into scientific research. Our analysis reveals a consistent pattern: LLMs meaningfully accelerate research workflows -- from hypothesis generation and literature synthesis to data analysis and scientific writing -- while introducing serious challenges related to hallucination, reproducibility, dataset bias, and model opacity. Beyond technical limitations, we identify ten underexplored challenges, including the erosion of researcher autonomy, AI-driven confirmation bias, authorship ambiguity, and unequal access to these technologies -- systemic risks that demand interdisciplinary governance frameworks, robust validation standards, and expanded explainability research.

==> sections/contributions.tex <==
\twocolumn[  
    \begin{@twocolumnfalse}
        \vspace{-1.24em}
        \section{Contributions and Acknowledgments}
     \end{@twocolumnfalse}
]

\enlargethispage{\baselineskip}

\textbf{Core Contributors} ($^*$: equal contributions)\\
Henrique Schechter Vera$^*$\\
Sahil Dua$^*$\\
Daniel Salz \\
Ryan Mullins \\
Sindhu Raghuram Panyam \\
Sara Smoot \\
Iftekhar Naim \\
Joe Zou \\
Feiyang Chen \\
Daniel Cer\vspace{1em}\\
\textbf{Contributors}\\
Alice Lisak \\
Min Choi \\
Lucas Gonzalez \\
Omar Sanseviero \\
Glenn Cameron \\
Ian Ballantyne \\
Kat Black \\
Kaifeng Chen \\
Weiyi Wang \\
Zhe Li \\
Gus Martins \\
Jinhyuk Lee \\
Mark Sherwood \\
Juyeong Ji \\
Renjie Wu \\
Jingxiao Zheng \\
Jyotinder Singh \\
Abheesht Sharma \\
Divyashree Sreepathihalli \vspace{0.5em}\\
\noindent\textbf{Gemini Embedding} \textit{(alphabetical order)}\\
Aashi Jain \\
Adham Elarabawy \\
AJ Co \\
Andreas Doumanoglou \\
Babak Samari \\
Ben Hora \\
Brian Potetz \\
Dahun Kim \\
Enrique Alfonseca \\
Fedor Moiseev \\
Feng Han \\
Frank Palma Gomez \\
Gustavo Hern{\'{a}}ndez {\'{A}}brego \\
Hesen Zhang \\
Hui Hui \\
Jay Han \\
Karan Gill \\
Ke Chen \\
Koert Chen \\
Madhuri Shanbhogue \\
Michael Boratko \\
Sai Meher Karthik Duddu \\
Sandeep Mariserla \\
Setareh Ariafar \\
Shanfeng Zhang \\
Shijie Zhang \\
Simon Baumgartner \\
Sonam Goenka \\
Steve Qiu \\
Tanmaya Dabral \\
Trevor Walker \\
Vikram Rao \\
Waleed Khawaja \\
Wenlei Zhou \\
Xiaoqi Ren \\
Ye Xia \\
Yichang Chen \\
Yi-Ting Chen \\
Zhe Dong \\
Zhongli Ding \vspace{0.5em} \\
\noindent\textbf{Gemma} \textit{(alphabetical order)}\\
Francesco Visin \\
Jiageng Zhang \\
Kathleen Kenealy \\
Michelle Casbon \\
Ravin Kumar \\
Thomas Mesnard \vspace{0.5em}\\
\noindent\textbf{T5Gemma} \textit{(alphabetical order)}\\
Biao Zhang \\
Ga\"{e}l Liu \\
Paul Suganthan \vspace{0.5em}\\
\noindent\textbf{Leadership}\\
Zach Gleicher \\
Cormac Brick \\
Olivier Lacombe \\
Adam Roberts \\
Qin Yin \\
Yunhsuan Sung \\
Raphael Hoffmann \\
Tris Warkentin \\
Armand Joulin \\
Tom Duerig \\
Mojtaba Seyedhosseini

\onecolumn
\noindent\textbf{Acknowledgement}\\
Daniel Estrada Alva, Krzysztof Czuba, Howard Zhou, Tom\'{a}\v{s} I\v{z}o, Tom Aarsen, Aditya Kusupati, Samer~Hassan, Aishwarya Nagarajan, Imed Zitouni
